ARCS: Agentic Retrieval-Augmented Code Synthesis with Iterative Refinement

We present Agentic Retrieval-Augmented Code Synthesis (ARCS), a system that improves LLM-based code generation without fine-tuning. ARCS operates through a budgeted synthesize-execute-repair loop over a frozen model: it retrieves relevant code context before generation, proposes candidates, executes them against tests, and repairs based on execution feedback. This retrieval-before-generation design reduces hallucination and accelerates convergence. We formalize ARCS as a state-action process with provable guarantees on termination, monotonic improvement, and bounded cost. A tiered controller (Small/Medium/Large) trades latency for accuracy predictably. On HumanEval, ARCS achieves up to 87.2% pass@1 with Llama-3.1-405B, surpassing CodeAgent (82.3%) while using simpler control than tree-search methods. On TransCoder, it achieves >= 90% accuracy on most translation pairs. On a LANL scientific corpus, it improves CodeBLEU by +0.115 over baseline RAG. ARCS provides a practical, reproducible approach to reliable code synthesis using existing LLM checkpoints.

==> del3.tex <==
\section{The ARCS Framework}
\label{sec:framework}

We present ARCS as a budgeted \emph{synthesize--execute--repair} loop that transforms a natural-language specification into a correct program using a frozen proposal model. This section unifies the theoretical formulation with its practical instantiation: each component is described with a clear formal specification and its implementation details.

\subsection{Overview and Core Loop}
\label{sec:framework:overview}

\begin{figure}[t] 
    \centering 
    \includegraphics[width=.85\linewidth]{iclr2026/Overview_agentic.pdf} 
    \caption{High-level overview of ARCS. (1) Extract and embed code snippets with metadata. (2) Use CoT planning to issue plan-conditioned retrieval queries; render retrieved evidence into the prompt. (3) Propose code, execute in a sandbox against tests, and encode execution feedback to repair iteratively.}
    \label{fig:agentic_overview} 
\end{figure} 

In each round, the controller: (i) \emph{retrieves} task-relevant code evidence to augment the prompt, (ii) \emph{synthesizes} a candidate (or edit) from a frozen model $\pi_{0}$ given the composed prompt, (iii) \emph{executes} it in a sandbox against a test suite to obtain verifiable feedback, and (iv) \emph{repairs} the prompt by encoding that feedback (and, when enabled, updating a plan and evidence). The process halts when all tests pass or a fixed iteration budget $B$ is exhausted.

\paragraph{Task and Notation.}
Given a natural-language specification $q$, the goal is to produce a program $\hat c^*$ that satisfies a test suite $\mathcal{T}=\{(x_i,y_i)\}_{i=1}^{m}$. We assume $m\ge1$ and treat any exception/timeout in the executor as a failure on the corresponding test. A candidate $\hat c$ is correct iff
\begin{equation}
\label{eq:correctness}
\hat c(x_i)=y_i \quad \forall i\in\{1,\ldots,m\}.
\end{equation}
We assume a code corpus $\mathcal{C}=\{c_1,\ldots,c_N\}$ with metadata $\mathcal{M}_i$ (signatures, docstrings, comments). For retrieval, we use an embedding function $\Phi:\ \mathcal{X}\to\mathbb{R}^d$ and denote $\mathbf{e}_i=\Phi(\mathcal{M}_i)$; in our implementation $\Phi$ is \texttt{all-MiniLM-L6-v2}.

\begin{algorithm}[t]
\caption{ARCS (Large Tier)}
\label{alg:arcs}
\begin{algorithmic}[1]
\Require spec $q$, test suite $\mathcal{T}$, budgets $k$ (retrieval), $B$ (iterations)
\Ensure program $\hat c^*$ (or best-so-far $\hat c^\star$)
\State $q_0 \gets q$;\ $s_0 \gets \varnothing$;\ $\hat c_0 \gets \varnothing$;\ $f_0 \gets \varnothing$
\For{$t = 0 \to B{-}1$}
  \State \textit{(optional CoT planning)} $s_t \gets P_\phi(q_t)$
  \State \textit{(retrieval)}
    \(
      \mathsf{R}_t \gets
      \begin{cases}
        \mathsf{Ret}_k(q_t), & s_t=\varnothing \\
        \mathrm{FilterRedundancy}\!\big(\!\bigcup_j \mathsf{Ret}_{k_j}(s_t^{(j)})\big), & \text{otherwise}
      \end{cases}
    \)
  \State \textit{(compose)} $q'_t \gets q_t \oplus \bigoplus_{c\in \mathsf{R}_t}\Psi(c)$
  \State \textit{(propose)} $\hat c_t \sim \pi_0(\cdot \mid q'_t)$
  \State \textit{(execute)} $f_t \gets \mathcal{E}(\hat c_t,\mathcal{T})$
  \If{$\hat c_t$ passes all tests} \State \Return $\hat c_t$ \EndIf
  \State \textit{(repair)} $q_{t+1} \gets q_t \oplus \mathrm{Encode}(f_t)$
\EndFor
\State \Return $\arg\max_{\hat c \in \{\hat c_0,\ldots,\hat c_{B-1}\}\setminus\{\varnothing\}}
        \sum_i \mathbf{1}[\hat c(x_i)=y_i]$
\end{algorithmic}
\end{algorithm}

\paragraph{Iterative Framework.}
We model one iteration using the tuple $(\mathcal{S},\mathcal{A},\mathcal{P},\mathcal{R})$:
\begin{itemize}
\item \textbf{State} $S_t=(q_t,s_t,\hat c_{t-1},f_{<t}) \in \mathcal{S}$ where $q_t$ is the current prompt/context, $s_t$ is an optional CoT plan, $\hat c_{t-1}$ is the previous candidate (or $\varnothing$ at $t=0$), and $f_{<t}$ are prior execution signals.
\item \textbf{Action} $A_t \in \mathcal{A}$ is the proposed code (or edit). In our instantiation, $A_t \equiv \hat c_t$ sampled from $\pi_0$.
\item \textbf{Transition} $\mathcal{P}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ executes the proposal in a sandbox and returns $S_{t+1}$ with updated context and feedback.
\item \textbf{Reward (optional)} $\mathcal{R}: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ measures improvement (e.g., the number of tests passed); used for selection/termination, not for weight updates.
\end{itemize}
The transition is
\begin{equation}
\label{eq:transition}
\hat c_t \sim \pi_{0}(\cdot\mid q'_t),\quad
f_t=\mathcal{E}(\hat c_t,\mathcal{T}),\quad
q_{t+1}=q_t\oplus \mathrm{Encode}(f_t),
\end{equation}
with halting rule
\begin{equation}
\label{eq:stop}
\text{halt if } \frac{1}{m}\sum_{i=1}^m \mathbf{1}[\hat c_t(x_i)=y_i]=1 \ \ \text{or}\ \ t=B-1.
\end{equation}
We track the best-so-far candidate as
\begin{equation}
\label{eq:bestsofar}
\hat c^\star_t \;=\; \arg\max_{\hat c\in\{\hat c_0,\ldots,\hat c_t\}\setminus\{\varnothing\}} \frac{1}{m}\sum_{i=1}^m \mathbf{1}[\hat c(x_i)=y_i].
\end{equation}

\paragraph{Design Guarantees.}
Termination is guaranteed after at most $B$ iterations by \Cref{eq:stop}; the best-so-far score in \Cref{eq:bestsofar} is non-decreasing in $t$ since the maximization set grows with $t$; and exact replay is enabled by fixing seeds, freezing the index snapshot, and using deterministic tie-breaking in retrieval (below).

\subsection{Core Components: Theory and Implementation}
\label{sec:framework:components}

\paragraph{Planner $P_\phi$.} 
\emph{Specification:} An optional CoT planner emits a plan $s_t=(s^{(1)}_t,\ldots,s^{(K)}_t)$, where each $s^{(j)}_t$ is a subgoal at iteration $t$. When unused, $s_t=\varnothing$ (i.e., $K=0$). \emph{Implementation:} A lightweight prompt produces (i) a typed I/O contract, (ii) a pseudocode sketch, and (iii) up to $K\leq 4$ named subgoals. We canonicalize symbols, deduplicate, and drop conflicts. A gate disables planning when $|q_t|<120$ tokens. Subgoal names are used directly as retrieval subqueries.

\paragraph{Retriever $R_\psi$.}
\emph{Specification:} 
Given $q_t$ (or subquery), embed $\phi_t=\Phi(q_t)$ and compute scores $\sigma_i=\mathrm{sim}(\phi_t,\mathbf{e}_i)$. Define the ordered index set
\begin{equation}
\label{eq:topk}
I_k(q_t)=\operatorname*{arg\,topK}_{i\in\{1,\ldots,N\}} \sigma_i
\quad\text{(ties broken deterministically by ascending index $i$)},
\end{equation}
and return
\begin{equation}
\label{eq:ret}
\mathsf{Ret}_k(q_t)=(c_{i_1},\ldots,c_{i_k})\ \ \text{with}\ \ (i_1,\ldots,i_k)=I_k(q_t).
\end{equation}
When $s_t\neq\varnothing$, define subqueries $q_t^{(j)}\coloneqq s_t^{(j)}$ and retrieve per component with budgets $k_j$:
\begin{equation}
\label{eq:subret}
\mathsf{Ret}_{k_j}(q_t^{(j)})=(c_{i^{(j)}_1},\ldots,c_{i^{(j)}_{k_j}}),
\end{equation}
then aggregate and deduplicate
\begin{equation}
\label{eq:aggret}
\mathsf{Ret}(q_t)=\mathrm{FilterRedundancy}\!\left(\bigcup_{j=1}^K \mathsf{Ret}_{k_j}(q_t^{(j)})\right).
\end{equation}
\emph{Implementation:} FAISS ANN index with cosine similarity over $\mathbf{e}_i$. Query with $q_t$ when $s_t=\varnothing$ or with $\{s^{(j)}_t\}$ otherwise, aggregate per \Cref{eq:aggret}. Near-duplicates are removed via cosine threshold ($\delta=0.85$); deprecated/conflicting APIs are filtered via a denylist. Snapshots are frozen for experiments.

\paragraph{Context Renderer and Proposer.}
\emph{Specification:} Render retrieved content via $\Psi : \mathcal{C} \to \mathcal{X}$:
\begin{equation}
\label{eq:render}
\Psi(c) = \mathrm{Format}(\mathrm{signature}(c), \mathrm{doc}(c), \mathrm{code}(c)),
\end{equation}
and compose the enriched prompt as
\begin{equation}
\label{eq:enriched}
q'_t \;=\; q_t \;\oplus\; \bigoplus_{c \in \mathsf{R}_t} \Psi(c),
\end{equation}
where $\mathsf{R}_t$ is produced either by single-query Top-$k$ (\Cref{eq:ret}) or by plan-conditioned retrieval with deduplication (\Cref{eq:aggret}). The frozen proposal model then generates
\begin{equation}
\label{eq:proposal}
\hat c_t \sim \pi_{0}(\cdot \mid q'_t).
\end{equation}
\emph{Implementation:} Frozen Llama-3.x checkpoints (\textit{Meta-Llama-3.1-70B/3.3-70B/3.1-405B Instruct}), nucleus sampling (temperature $0.7$, top-$p=0.95$, $L_{\max}=512$, seed $42$). Encoders: $\text{Enc}_{\text{env}}$ (runtime constraints), $\text{Enc}_{\text{plan}}$ (subtasks), $\text{Enc}_{\text{evid}}$ (retrieved code), $\text{Enc}_{\text{inv}}$ (interface invariants).

\paragraph{Executor $\mathcal{E}$.}
\emph{Specification:} Execute $\hat c_t$ w.r.t.\ $\mathcal{T}$:
\begin{equation}
\label{eq:exec}
f_t = \mathcal{E}(\hat c_t, \mathcal{T}).
\end{equation}
\emph{Implementation:} Docker sandbox (no network; read-only FS except a temp workspace). Per-test caps: 10s wall-clock, 4GB memory. We capture exit codes, stdout/stderr, and exception metadata. $\text{Enc}_{\text{fb}}$ serializes pass/fail vectors and truncated stacks.

\paragraph{Repair and Refresh.}
\emph{Specification:} Append feedback and optionally re-plan:
\begin{equation}
\label{eq:update}
q_{t+1}=q_t \oplus \mathrm{Encode}(f_t), \qquad s_{t+1}=P_\phi(q_{t+1}; s_t, f_t).
\end{equation}
Refresh evidence under the updated query:
\begin{equation}
\label{eq:refresh}
\mathsf{Refresh}(q_{t+1},s_{t+1}) \triangleq
\begin{cases}
\mathsf{Ret}_k(q_{t+1}) & \text{if } s_{t+1}=\varnothing,\\[2pt]
\mathrm{FilterRedundancy}\Big(\bigcup_{j=1}^{K} \mathsf{Ret}_{k_j}(s_{t+1}^{(j)})\Big) & \text{otherwise.}
\end{cases}
\end{equation}
\emph{Implementation:} $\text{Enc}_{\text{fb}}$ summarizes only \emph{observed} failures (exception type, failing inputs, truncated stack). On context pressure, apply stable truncation: keep $\text{Enc}_{\text{inv}}$ and the most recent failing trace; drop lowest-similarity evidence first; collapse $\text{Enc}_{\text{plan}}$ to headers.

\subsection{Theoretical Properties and Guarantees}
\label{sec:framework:theory}

\begin{proposition}[Monotonic Improvement]
\label{prop:monotonic}
Under best-so-far tracking (\Cref{eq:bestsofar}), the success metric is non-decreasing:
\[
\forall t:\quad \frac{1}{m}\sum_{i=1}^m \mathbf{1}[\hat c^\star_{t+1}(x_i)=y_i] 
\;\geq\; \frac{1}{m}\sum_{i=1}^m \mathbf{1}[\hat c^\star_t(x_i)=y_i].
\]
\end{proposition}
\begin{proof}
$\{\hat c_0,\ldots,\hat c_{t+1}\}\setminus\{\varnothing\} \supseteq \{\hat c_0,\ldots,\hat c_t\}\setminus\{\varnothing\}$, so the maximized value cannot decrease.
\end{proof}

\begin{proposition}[Bounded Termination]
\label{prop:termination}
Algorithm~\ref{alg:arcs} terminates in at most $B$ iterations.
\end{proposition}
\begin{proof}
The loop runs for $t=0,\ldots,B-1$ with an early return when all tests pass (\Cref{eq:stop}); hence termination is guaranteed after at most $B$ iterations.
\end{proof}

\begin{proposition}[Cost Bound]
\label{prop:cost}
Let $C_{\text{retr}}(k)$ bound the per-round retrieval cost (including ANN probes and formatting of the top-$k$ items), 
$C_{\text{in}}(L)$ and $C_{\text{out}}(L)$ bound the LLM's input and output token costs for length $L$, 
and $C_{\text{exec}}$ bound the per-test execution cost in $\mathcal{E}$. 
If $|q'_t|\le L_{\max}$ and $\hat c_t$ has at most $L_{\max}$ output tokens each round, then
\begin{equation}
\label{eq:cost}
C_{\text{total}} \;\le\; B \cdot \big( C_{\text{retr}}(k) + C_{\text{in}}(L_{\max}) + C_{\text{out}}(L_{\max}) + m \cdot C_{\text{exec}} \big).
\end{equation}
\end{proposition}
\begin{proof}
Each round incurs retrieval, LLM input/output, and up to $m$ test executions. Upper-bounding each term and summing over at most $B$ rounds yields the result.
\end{proof}

\begin{lemma}[Tier Monotonicity]
\label{lem:tier}
Fix the backbone $\pi_0$, corpus/index, and benchmark distribution. 
Define the attainable success probability of a tier as the supremum over its controller parameters and internal randomness.
Then $\mathcal{P}_S \le \mathcal{P}_M \le \mathcal{P}_L$.
\end{lemma}
\begin{proof}
Small is the subset of controllers with $(k=0,\, s_t=\varnothing,\, B=1)$. 
Medium enlarges this set to allow $s_t\neq\varnothing$ but keeps $(k=0,\,B=1)$. 
Large further enlarges to $k>0$ and $B>1$. 
Since each controller class is a subset of the next, the supremum success over a subset is at most that over its superset.
\end{proof}

\subsection{Tier Design and Operational Modes}
\label{sec:framework:tiers}

We expose a tiered interface to provide predictable accuracy--latency trade-offs and enable clean ablations. Each tier is a strict projection of the full controller, preserving the guarantees above:
\begin{itemize}
\item \textbf{Small (one-shot):} No planning or retrieval, one round—$(k=0, s_t=\varnothing, B=1)$. Compose, propose, test.
\item \textbf{Medium (structured single-shot):} Planning enabled, retrieval disabled, one round—$(k=0, s_t\neq\varnothing, B=1)$. Exploits decomposition when specifications are complete.
\item \textbf{Large (retrieval+repair):} Planning, plan-conditioned retrieval with refresh, multi-round repair—$(k>0, s_t\neq\varnothing, B>1)$.
\end{itemize}
Default parameters: $k=10$ (retrieval budget), $B=5$ (iteration budget), $K\leq 4$ (max subgoals). Since higher tiers can emulate lower ones by setting parameters to zero, attainable success probability is non-decreasing across tiers.

\subsection{System Implementation and Reproducibility}
\label{sec:framework:implementation}

The ARCS system runs on the SambaNova Systems platform with real-time LLM API access. The framework is modular Python code that queries live code repositories for retrieval; for experiments we freeze snapshots by embedding metadata offline and indexing it to avoid runtime drift.

Determinism/replay: versioned LLM checkpoints and FAISS indices, fixed seeds and decoding hyperparameters, and complete logging of $(q_t,s_t,q'_t,\hat c_t,f_t)$ per round with index snapshots, enabling full replay of the transition dynamics in \Cref{eq:transition}.
